Performance forecasts for the primordial gravitational wave detection pipelines for AliCPT-1

AliCPT is the first Chinese cosmic microwave background (CMB) experiment which will make the most precise measurements of the CMB polarization in the northern hemisphere. The key science goal for AliCPT is the detection of primordial gravitational waves (PGWs). It is well known that an epoch of cosmic inflation, in the very early universe, can produce PGWs, which leave an imprint on the CMB in form of odd parity $B$-mode polarization. In this work, we study the performance of the component separation and parameter estimation pipelines in context of constraining the value of the tensor-to-scalar ratio. Based on the simulated data for one observation season, we compare five different pipelines with different working principles. Three pipelines perform component separation at map or spectra level before estimating $r$ from the cleaned spectra, while the other two pipelines performs a global fit for both foreground parameters and $r$. We also test different methods to account for the effects of time stream filtering systematics. This work shows that our pipelines provide consistent and robust constraints on the tensor-to-scalar ratio and a consistent sensitivity $\sigma(r) \sim 0.02$. This showcases the potential of precise $B$-mode polarization measurement with AliCPT-1. AliCPT will provide a powerful opportunity to detect PGWs, which is complementary with various ground-based CMB experiments in the southern hemisphere.

==> cpt_violation.tex <==
The temperature and polarization anisotropies of the CMB
radiation are powerful cosmological observables to understand the physics of the early universe. During the past decades, much effort has been made to characterize the CMB, including three satellite generations: the cosmic background explorer (COBE), the Wilkinson
microwave anisotropy probe (WMAP) and Planck. These experiments were mainly devoted
to measure the CMB temperature anisotropies, precisely mapping these tiny fluctuations in
the sky. However, according to the standard cosmological model, the full information
of CMB is encoded in the statistical properties of both temperature, $T(\hat{\gamma})$, and the linear
polarizations, described by the stocks parameters, $Q(\hat{\gamma})$ and $U(\hat{\gamma})$, which are defined with respect to a fixed coordinate system in the sky, and depend on the choice of coordinate system.
It is then convenient to decompose the linear polarization into the curl-free ($E$-mode) and
divergence-free ($B$-mode) components since they have the advantage of being rotationally
invariant. Recent results from the Planck satellite also show precise measurements of the $E$-mode
field. In the standard cosmological model, both CMB temperature and $E$-mode
anisotropies are mainly generated by the primordial density perturbations. In addition, the
auto-correlation power spectra $C_{\ell}^{TT}$
and $C_{\ell}^{EE}$ and the cross-correlation power spectrum $C_{\ell}^{TE}$
sensitively depend on the cosmological parameters and cosmological models. Thus, the observations of WMAP and Planck satellites on these spectra have tightly constrained most
cosmological parameters and inflationary parameters. However, the $B$-mode polarization encodes quite different cosmological information: in the large scales, the $B$-mode polarization
is supported to be generated by the primordial gravitational waves, which is
the smoking-gun evidence of inflation. In the small scales, the $B$-mode is mainly
produced by the deflection of the CMB photons by cluster of galaxies during their travel
between the last scattering surface and the observer, known as the CMB lensing. In addition, the CMB $B$-mode polarization also provides an excellent opportunity to the test the fundamental physical laws. For instance, if the CPT symmetry is violated during the evolution of the Universe for some reasons, the cosmic birefringence effect can occur, which induces the nonzero   
correlation power spectra $C_{\ell}^{TB}$ and $C_{\ell}^{EB}$. Therefore, the measurement of these two spectra can be used to the test CPT symmetry in the cosmological scales.


In the post-Planck era, various ground-based CMB experiments, including BICEP, Keck Array, PolarBear, SPT, ACT, CMB S4 project and so on.
In the near future, AliCPT is the unique CMB experiment in the northern hemisphere, which is complementary to the CMB telescopes south pole or Chile. The main science goal of AliCPT is to observe the CMB polarizations, in particular the $B$-mode polarization, with high precision in the northern hemisphere for the first time. By analyzing these observables, one can detect the primordial gravitational waves, the cosmic weak lensing, and test the CPT symmetry. In the real observations, the CMB $B$-mode polarization is contaminated by many sources, including the instrumental noises, various foreground emissions, the $E$-$B$ mixture due to the partial sky observations, and various systematics. In the article, ......................................

\section{Forecasts on CPT rotation angle (Chang, Zhai-Hua)}
\label{sec:forecast_cpt}
If the CMB photons were coupled to a pseudo-scalar field $\phi$ during the propagation via the so-called Chern-Simons (CS) term that is described as 

\begin{equation}\label{coupling}
\mathcal{L}_{\rm CS}= \partial_{\mu}f(\phi)A_{\nu}\tilde{F}^{\mu\nu}~,
\end{equation}
where $f$ is an arbitrary function of $\phi$, this coupling would imply that the CS term violates Lorentz and CPT symmetries and can slightly rotate the Stokes parameters $Q$ and $U$ by a rotation angle $\alpha$ as
\begin{equation}
Q'\pm iU'=(Q\pm iU)e^{\pm i2\alpha}.\label{qurot}
\end{equation}

The rotation angle corresponds to the CPT violation and is frequency independent. The accumulated rotation angle along the line of sight is given by~\cite{2008PhRvD..78j3516L}
\begin{equation}\label{ro}
\alpha=\int^s_o\partial_{\mu}f(\phi) dx^{\mu}(\lambda)=f(\phi_s)-f(\phi_0)~,
\end{equation}
once the evolution of the scalar field is determined with a given potential $V(\phi)$. The result indicates that the nonvanishing rotation angle arises from different values of the scalar fields at both the last scattering surface and today. 


The stokes parameters $Q$ and $U$ can be decomposed into electric-like and curl-like modes, i.e., $E$ and $B$ modes. Likewise, the observed $E$ and $B$ modes are rotated by the angle $\alpha$ as 
\begin{eqnarray}
E({\bf l})&=&\cos{(2\alpha)} \tilde E({\bf l}) - \sin{(2\alpha)} \tilde B({\bf l}) \nonumber \\
B({\bf l})&=&\sin{(2\alpha)} \tilde E({\bf l}) + \cos{(2\alpha)} \tilde B({\bf l})\,.
\end{eqnarray}
Due to the rotation, a new type of B-mode is created even if the primordial B mode is zero. Consequently, all the CMB power spectra modified by the rotation angle are expressed as
\begin{eqnarray}
C^{TE}_\ell  &= &\cos{(2\alpha)} \tilde {C}^{TE}_\ell \nonumber \\
C^{EE}_\ell&=&\sin^2{(2\alpha)} \tilde C^{BB}_{\ell} + \cos^2{(2\alpha)} \tilde C^{EE}_{\ell} \nonumber \\
C^{EB}_\ell&=&\frac{1}{2}\sin{(4\alpha)} (\tilde C^{BB}_\ell - \tilde C^{EE}_{\ell}) \nonumber \\
C^{TB}_\ell&=&\sin{(2\alpha)} \tilde C^{TE}_\ell \nonumber \\
C^{BB}_\ell&=&\cos^2{(2\alpha)} \tilde C^{BB}_\ell + \sin^2{(2\alpha)} \tilde C^{EE}_\ell\,.
\label{eq:spectra}
\end{eqnarray}
The above equations indicate that a rotation angle can be inferred from the nonvanishing power spectra $C_{\ell}^{TB}$ and $C_{\ell}^{EB}$, which are originally null due to symmetry requirement. The inferred rotation angle is of great importance in that it could hint existence of the exotic scalar field if there were no other sources of polarization rotations. On the other hand, the rotation angle can be decomposed into a constant and an anisotropic components, i.e., $\alpha ({\bf n})=\alpha_0+\Delta\alpha({\bf n})$.There are different methods to extract both the constant rotation~\cite{2006PhRvL..96v1302F,2007PhLB..651..357L} and the anisotropic ones~\cite{2009PhRvL.102k1302K}. The first rotation angle measurement was made using the WMAP and the 2003 BOOMERANG datasets ~\cite{2006PhRvL..96v1302F}. Subsequently, there were a plethora of measurements showing evidence of nonzero rotation angles from various CMB datasets. 

A nonzero rotation angle can not only produce TB and EB correlations, but also transfer power from the primordial $\tilde C^{EE}_\ell$ to the $B$-mode power spectra, contaminating the $B$-mode signal from the primordial gravitational waves that are quantified by the tensor-to-scalar ratio $r$. 
\begin{figure}
    \centering
    \includegraphics[width=0.48\textwidth]{figures/ebhalfdeg.png}
        \caption{Rotation-induced B-mode power spectrum with $\beta=0.5^{\circ}$. }
    \label{ebrot}
\end{figure}
In addition to the cosmological origin of the rotation angle ($\beta$), polarization angle miscalibration of detector pixels can also give rise to a nonzero rotation angle $\alpha$ that is degenerate with the former. This necessitates a de-rotation procedure to eliminate the miscalibration angle. To this end, the self-calibration approach\cite{2013ApJ...762L..23K} was proposed. Presumably, the cosmic rotation is secondary to the miscalibration, thus the self-calibration works well in terms of systematic mitigations. However, the cosmic rotation angle would not survive after the self-calibration procedure, complicating its measurements.

To decouple the degeneracy between the cosmic rotation $\beta$ and miscalibration $\alpha$, a novel approach was recently developed in~\cite{2019arXiv190412440M}, where the polarized foreground is used to break the degeneracy. The method is built upon the fact that the CMB is rotated by both the scalar field and miscalibration, but the polarized emission from the Galactic foreground is mainly rotated by the miscalibration angle. The observed $E$ and $B$ modes which contain both components now become
\begin{eqnarray}
E({\bf l})&=&\cos{(2\alpha)} \tilde E^{\rm fg}({\bf l}) - \sin{(2\alpha)} \tilde B^{\rm fg}({\bf l})+\cos{(2\alpha+2\beta)} \tilde E^{\rm CMB}({\bf l}) - \sin{(2\alpha+2\beta)} \tilde B^{\rm CMB}({\bf l})\nonumber \\
B({\bf l})&=&\sin{(2\alpha)} \tilde E^{\rm fg}({\bf l}) + \cos{(2\alpha)} \tilde B^{\rm fg}({\bf l})+\sin{(2\alpha+2\beta)} \tilde E^{\rm CMB}({\bf l}) + \cos{(2\alpha+2\beta)} \tilde B^{\rm CMB}({\bf l})\,,
\end{eqnarray}

and the corresponding EB correlation becomes
\begin{equation}
\begin{split}
\langle C_\ell^{EB,\mathrm{o}}\rangle =&
\frac{\tan(4\alpha ) }{2}
\left(\langle C_\ell^{EE,\mathrm{o}}\rangle-\langle C_\ell^{BB,\mathrm{o}}\rangle\right)
+
\frac{\sin(4\beta)}{2\cos(4\alpha)}\left(
\langle C_\ell^{EE,\mathrm{CMB}}\rangle - \langle C_\ell^{BB,\mathrm{CMB}}\rangle
\right)\\
&+\frac1{\cos(4\alpha)}\langle C_\ell^{EB,\mathrm{fg}}\rangle
+\frac{\cos(4\beta)}{\cos(4\alpha)}\langle C_\ell^{EB,\mathrm{CMB}}\rangle\,.
\end{split}\label{GeneralRotationFitting}
\end{equation}

Using Eq. (\ref{GeneralRotationFitting}), we can construct the likelihood function for both angles as
\begin{equation}
-2\ln \mathcal{L}
= \sum_{\ell=\ell_\mathrm{min}}^{\ell_\mathrm{max}}
\frac{
\left[
C_\ell^{EB,\mathrm{o} } 
- \frac{\tan(4\alpha) }{ 2 }  \left( C_\ell^{EE,\mathrm{o} } - C_\ell^{ BB,\mathrm{o} } \right)
-  \frac{ \sin(4\beta) }{ 2\cos( 4\alpha ) }
\left(
C_{\ell}^{EE,\mathrm{CMB} } - C_{\ell}^{BB,\mathrm{CMB} } 
\right)
\right]^2
}{
{\rm Var} \left[
C_\ell^{ EB, \mathrm{o} } - \frac{\tan(4\alpha) }{ 2 }  \left( C_\ell^{EE,\mathrm{o} } - C_\ell^{ BB,\mathrm{o} } \right)
\right]
}.\label{LikelihoodGeneral}
\end{equation}


A CMB experiment with a large sky coverage would become advantageous in that it can cover regions with different polarized foregrounds. This makes AliCPT a perfect experiment for studying the rotation angles, and we adopt the new approach Eq. (\ref{LikelihoodGeneral}) to estimate uncertainties of the rotation angle using the first-year observations. 
\begin{figure}
    \centering
    \includegraphics[width=0.48\textwidth]{figures/polnoise.png}
    \caption{Polarization noise depths at 95 and 150GHz.}
    \label{fig:polnoise}
\end{figure}
We consider two frequencies 95 and 150GHz with $19'$ and $12'$ FWHM for the first-year observations. The polarization noise depths after one-year scanning are shown in Figure \ref{fig:polnoise}, and median depth values are found to be $\sim17\mu K-arcmin$ and $\sim 25\mu K-arcmin$ for 95 and 150GHz, respectively. The sky coverage is about 10\%. We choose the multipole range $32<\ell<1052$ for the forecasts. 

We generate Gaussian realizations for the underlying CMB sky and run PySM to generate templates of synchrotron and thermal dust. The power spectra for the foreground are shown in Figure \ref{polps}.
\begin{figure}
    \centering
    \includegraphics[width=1\textwidth]{figures/pol_fg.png}
    \caption{Power spectra of the polarized foreground.}
    \label{polps}
\end{figure}

We include no rotation angle in the analysis and apply the novel method described in Eq. (\ref{LikelihoodGeneral}) to the mock power spectra $C_{\ell}^{EB}$. The first-year upper bound is $\Delta\beta<0.6^\circ$, whereas $\Delta(\alpha+\beta)\sim\mathcal O(0.01^\circ)$ if the overall angle is considered and the self-calibration is applied.
\begin{figure}
    \centering    \includegraphics[width=0.48\textwidth]{figures/alicpt_cbangle.png}
    \caption{Posterior distribution of the cosmic rotation angle.}
    \label{alicptaa}
\end{figure}


The cosmic rotation can also induce higher-order correlations which might provide complementary limits as well. Ref. \cite{2020JCAP...12..051Z} recently found that a 0.1 deg level rotation can introduce noticeable differences on the CMB bispectra. The B mode polarization from AliCPT will enhance the detectability of the cosmic rotation and better constrain the Chern-Simons theory.
\begin{eqnarray}
B_{l_1l_2l_3}^{m_1m_2m_3} &=& \langle a^X_{l_1m_1} a^Y_{l_2m_2}a^Z_{l_3m_3}\rangle =  \left( {\begin{array}{ccc}
l_1 &l_2 & l_3 \\
m_1 & m_2 & m_3\\
\end{array} } \right)B_{l_1l_2l_3}^{XYZ},
\end{eqnarray}
